Minimal-Variance Distributed Deadline Scheduling

Many modern schedulers can dynamically adjust their service capacity to match the incoming workload. At the same time, however, unpredictability and instability in service capacity often incur operational and infrastructure costs. In this paper, we seek to characterize optimal distributed algorithms that maximize the predictability, stability, or both when scheduling jobs with deadlines. Specifically, we show that Exact Scheduling minimizes both the stationary mean and variance of the service capacity subject to strict demand and deadline requirements. For more general settings, we characterize the minimal-variance distributed policies with soft demand requirements, soft deadline requirements, or both. The performance of the optimal distributed policies is compared to that of the optimal centralized policy by deriving closed-form bounds and by testing centralized and distributed algorithms using real data from the Caltech electrical vehicle charging facility and many pieces of synthetic data from different arrival distribution. Moreover, we derive the Pareto-optimality condition for distributed policies that balance the variance and mean square of the service capacity. Finally, we discuss a scalable partially-centralized algorithm that uses centralized information to boost performance and a method to deal with missing information on service requirements.

==> 2018_OR_ deadline scheduling (new May 28) (1)/macro_new.tex <==
\usepackage{amsfonts,amssymb,amsmath} 
%\usepackage{subfigure}
\usepackage{mathtools}
\usepackage{tikz}
\usepackage{url}
\usetikzlibrary{external,matrix,fit,external,arrows}
\usepackage{pgfplots}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[toc,page]{appendix}


% define symbols
\newcommand{\hV}{\mathcal{V}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\hT}{\mathcal{T}}
\newcommand{\hF}{\mathcal{F}}
\newcommand{\hS}{\mathcal{S}}
\newcommand{\hI}{\mathcal{I}}





\newcommand{\he}{\hat \sigma}

\newcommand{\U}{U}
\newcommand{\hh}{h}

\newcommand{\card}{\text{card}}
\newcommand{\len}{\text{len}}
\newcommand{\real}{\mathbb R}

% ENGLISH
\newcommand{\eg}{\textit{e.g. }}
\newcommand{\ie}{\textit{i.e. }}

% % SYMBOLS: Yorie 
% \newcommand{\at}{a}
% \newcommand{\e}{e}
% \newcommand{\rate}{r}
% \newcommand{\p}{P}
% \newcommand{\st}{x}
% \newcommand{\x}{x}% remaining time 
% \newcommand{\dd}{d}


% JOB PROFILES 
\newcommand{\at}{a}		% arrival time
\newcommand{\e}{\sigma}		% demand
\newcommand{\p}{P}			% service capacity
\newcommand{\rate}{r}
\newcommand{\st}{\tau}		% sojourn time
\newcommand{\hst}{\hat \tau}	% extended sojourn time
\newcommand{\x}{y}			% remaining time 
\newcommand{\y}{x}			% remaining demand
\newcommand{\dd}{d}		% deadline 




% SCHEDULING POLICY
\newcommand{\uc}{c}		% scheduling policies for lower bound
\newcommand{\uind}{\bar u}
\newcommand{\off}{o}		% scheduling policies for lower bound

% OPTIMIZATION PROBLEMS 
\newcommand{\C}{\delta}	
\newcommand{\D}{\epsilon}
\newcommand{\Q}{W}
\newcommand{\Ph}{\eqref{eq:cost2}}	
\newcommand{\Ps}{\eqref{eq:cost2}}	
\newcommand{\YDS}{\eqref{eq:YDS_optimization_problem}}


\newcommand{\hp}{\tilde v}	

% sets 
\newcommand{\Z}{\mathbb Z_+}
\newcommand{\R}{\mathbb R}
\newcommand{\Rp}{\mathbb R_+}
% probability
\newcommand{\pro}{\mathbb{P}}
\newcommand{\pois}{\Psi}
\newcommand{\pspace}{A}
\newcommand{\pint}{\Lambda}
\newcommand{\pinti}{\Lambda}
\newcommand{\fint}{\lambda}
\newcommand{\N}{N}

% optimization problem
\newcommand{\opts}{\mathcal P}

